Global Observability Analysis of a Growth Model for Insects Farming

The Hermetia illucens insects or the black soldier fly has been attracting a growing interest in the food and feed industry. For its high nutritional value on the one hand, and because it is an adequate species for insects in controlled environmental agriculture systems, on the other. Therefore, several models describing this larvae's behaviour have been developed in the literature. Due to the complex nature of living organisms, systems of controlled environment agriculture are characterised by their strong nonlinearities. In this paper, we present a three dimensional nonlinear model describing the black soldier fly dry biomass weight dynamic changes due to the temperature's influence. In practice, this biomass weight is not measured in real time. This becomes problematic for applying feedback control strategies that assume full information of the states. Thus, this work investigates the observability of the dry biomass of a Hermetia illucens farming batch. The instantaneous and global observability of the aforementioned model is proven by constructing an injective transformation between the state space and a higher dimensional space where the transformed states are observable.

==> ACSD_CR_preamble.tex <==
%%%%% ACSD CR Preamble START %%%%%

\newcommand{\ACC}[2]{This work has been accepted in the {#1}, {#2}}

\newcommand{\CRIEEE}{©\the\year IEEE. Personal use of this material is permitted. Permission from IEEE must be obtained for all other uses, in any current or future media, including reprinting/republishing this material for advertising or promotional purposes, creating new collective works, for resale or redistribution to servers or lists, or reuse of any copyrighted component of this work in other works.}

\newcommand{\CRELSE}[1]{©\the\year. This manuscript version is made available under the CC-BY-NC-ND 4.0 license {#1}}

\newcommand{\CRIFAC}[2]{©\the\year { #1}. This work has been accepted to IFAC for publication under a Creative Commons Licence CC-BY-NC-ND {#2}}

%%%%% ACSD CR Preamble END %%%%%
